Prompt-augmented Temporal Point Process for Streaming Event Sequence

Neural Temporal Point Processes (TPPs) are the prevalent paradigm for modeling continuous-time event sequences, such as user activities on the web and financial transactions. In real-world applications, event data is typically received in a \emph{streaming} manner, where the distribution of patterns may shift over time. Additionally, \emph{privacy and memory constraints} are commonly observed in practical scenarios, further compounding the challenges. Therefore, the continuous monitoring of a TPP to learn the streaming event sequence is an important yet under-explored problem. Our work paper addresses this challenge by adopting Continual Learning (CL), which makes the model capable of continuously learning a sequence of tasks without catastrophic forgetting under realistic constraints. Correspondingly, we propose a simple yet effective framework, PromptTPP\footnote{Our code is available at {\small \url{ https://github.com/yanyanSann/PromptTPP}}}, by integrating the base TPP with a continuous-time retrieval prompt pool. The prompts, small learnable parameters, are stored in a memory space and jointly optimized with the base TPP, ensuring that the model learns event streams sequentially without buffering past examples or task-specific attributes. We present a novel and realistic experimental setup for modeling event streams, where PromptTPP consistently achieves state-of-the-art performance across three real user behavior datasets.

==> chapters/_relatedwork.tex <==

\section{Related work}\label{sec:related}
Here we draw connections and discuss differences between our method to related works. Due to the page limit, please see \cref{app:related} for a more detailed discussion.

\textbf{Temporal Point Process.} A large variety of Neural TPPs \citep{du-16-recurrent,mei-17-neuralhawkes,xiao-17-modeling,omi-19-fully,shchur-20-intensity,mei-2020-datalog,boyd-20-vae} have been proposed over recent decades, aimed at modeling event sequences with varying sorts of properties. To the best of our knowledge, there exist two prior works \cite{yang-2017-omhp,eric-2016-track} that propose online learning algorithms for classical TPPs while that for neural TPP have rarely been studied. We show our method works better than classical online TPPs in practice (see \cref{sec:main_result}). 


\textbf{Continual Learning.}
There is also a rich existing literature on CL \citep{kirkpatrick2017overcoming,zenke2017continual,rusu2016progressive}. In retrospect, we realize a concurrent work \citep{dubey-2022} which augments TPP with CL abilities. Important distinctions of their work from ours include: 1. setup: they use standard TPP train/valid setting while we formalize a more realistic streaming setting to train/validate the models; 2. methodology: they model the event streams with a hypernetwork-based regularizer while we use a trainable prompt pool with more flexibility and generality in CL. 3. task agnostic: they rely on a task descriptor built from meta attributes of events while we do not - our method is task agnostic. We show that our method outperforms it (see \cref{sec:main_result}). 

\textbf{Prompt Learning.} Prompt-based learning (or prompting) \citep{lester2021power,li2021prefix},  applies a fixed function to condition the model, so that the language model gets additional instructions to perform the downstream task. \citet{wang2022dualprompt,wang2022learning} connect prompting and CL, which attaches prompts to the pretrained backbone to learn task-invariant and task-specific instructions. Note
that it is non-trivial to apply prompting to neural TPPs (See Analysis II,III in \cref{sec:main_result}) and our proposed novel framework reveals its values to event sequence modeling.
